SINET: Sparsity-driven Interpretable Neural Network for Underwater Image Enhancement

Improving the quality of underwater images is essential for advancing marine research and technology. This work introduces a sparsity-driven interpretable neural network (SINET) for the underwater image enhancement (UIE) task. Unlike pure deep learning methods, our network architecture is based on a novel channel-specific convolutional sparse coding (CCSC) model, ensuring good interpretability of the underlying image enhancement process. The key feature of SINET is that it estimates the salient features from the three color channels using three sparse feature estimation blocks (SFEBs). The architecture of SFEB is designed by unrolling an iterative algorithm for solving the $\ell_1$ regularized convolutional sparse coding (CSC) problem. Our experiments show that SINET surpasses state-of-the-art PSNR value by $1.05$ dB with $3873$ times lower computational complexity. Code can be found at: https://github.com/gargi884/SINET-UIE/tree/main.

==> images/fig_lsui.tex <==
\begin{figure*}[hbt!] 
    \centering
  {\includegraphics[width=\linewidth]{images/sota_lsui.png}}
  \caption{More visual comparison with SOTA methods for images from the LSUI dataset. Our proposed SINET presereves the object colors and structure more accurately and resemble more similar to the ground truth images. Images are best viewed in $400\%$ zoom.}
  \label{figlsui} 
\end{figure*}

==> images/fig_uiebc.tex <==
\begin{figure*}[hbt!] 
    \centering
  {\includegraphics[width=\linewidth]{images/sota_uiebc.png}}
  \caption{More visual comparison with SOTA methods for images from the UIEBC dataset. Our proposed SINET presereves the object colors and structure more accurately. Images are best viewed in $400\%$ zoom.}
  \label{figuiebc} 
\end{figure*}

==> sec/0_abstract.tex <==
\begin{abstract}
In recent years, deep learning-based methods have achieved impressive results
in underwater image enhancement (UIE). However, these methods often lack
interpretability, making it difficult to understand the enhancement process. To
address this issue, we introduce MINet, a model-based interpretable network
designed for UIE. MINet is built on a novel channel-specific convolutional sparse coding (CCSC) model.
MINet first estimates the sparse features from the different color channels using sparse feature estimation blocks (SFEBs) and then gets the enhanced color channels from these sparse features. Specifically, with an $\ell_1$ regularized formulation, SFEBs constrain the sparse features to be of low noise levels. Our experiments show that with a very low computational complexity, MINet surpasses state-of-the-art methods in performance. Models and code can be found at the following link: [Link]
\end{abstract}
%
\begin{keywords}
Underwater image enhancement, channel-specific convolutional sparse coding, interpretable network.
\end{keywords}

==> sec/1_intro.tex <==
\input{images/fig1}
\section{Introduction}
\label{sec:intro}
Underwater images are essential for various applications, such as marine
biology research, underwater archaeology, and resource management.
However, these images often suffer from severe degradation due to the
absorption and scattering of light in underwater environments. The attenuation
of light is non-uniform across different color channels, exacerbating the issue.
To address these challenges and enhance the usability of underwater images for
high-level vision tasks, numerous underwater image enhancement (UIE)
techniques \cite{uieb,uiewd,scnet,deepwavenet,FUnIEGAN,x_caunet,DSFFNet} have been developed.  Recent methods \cite{deepwavenet,x_caunet} have employed deep neural networks specifically designed for
UIE, considering the non-uniform attenuation of different color wavelengths.
These color channel-specific designs have proven to be highly effective for
UIE. Despite the potential of deep learning (DL)--based methods to learn
complex mappings between degraded and enhanced images, they often lack
interpretability regarding the underlying image enhancement process \cite{unrolling, urolling_boyd}. This
limitation highlights the need for approaches that not only improve image
quality but also provide a clear understanding of the enhancement mechanisms
involved.

To incorporate interpretability in the network architecture, Sreter \textit{et al.} \cite{lcsc} used a convolutional sparse coding (CSC) model-based network design for denoising of ordinary images. Given the degraded source image $I_s\in\mathbb{R}^{H \times W \times 3}$, \cite{lcsc} expressed it using convolutional sparse representations $z\in\mathbb{R}^{H \times W \times K}$ as,
\begin{equation}\label{eq1}
    I_s = D(z)
\end{equation}

where $D(\cdot)$ is convolutional dictionary which can be learned, and $K$ is number of convolution filters. Eqn. \ref{eq1} is formulated as an $\ell_1$ regularized optimization problem for constraining $z$ with low noise level,

\begin{equation}\label{l11}
\underset{z}{\mathrm{Argmin}}\:\frac{1}{2}\Big|\Big|\:I_{s}-D(z)\Big|\Big|_2^2 +\lambda ||z||_1 
\end{equation}

For solving Eqn. \ref{l11}, \cite{lcsc} proposed a learned convolutional sparse coding (LCSC) block by unrolling the steps of the iterative shrinkage thresholding algorithm (ISTA) \cite{ista}. However, \cite{lcsc} did not consider the color channel-dependent degradation scenario, which is important in underwater images. Also, there is some room for improvement in the LCSC block.

In this work, we propose a novel channel-specific convolutional sparse coding (CCSC) model to represent the UIE process by considering the wavelength-dependent degradation in underwater images. Based on this CCSC model, we propose MINet, a deep network for the UIE task. Due to this model-based design, the architecture of MINet has the interpretability of the image enhancement process.
 Specifically, we propose a sparse feature estimation block (SFEB) by modifying the LCSC block \cite{lcsc} to estimate the sparse features from the different color channels. Following this estimation step, the enhanced images for each color channel are restored, which are finally concatenated to get the final enhanced image. 
 Our contributions can be summarized as,

 \begin{itemize}
 \item  We propose a novel channel-specific convolutional sparse coding (CCSC) model for the UIE process. In this model, we consider the channel-dependent degradation in underwater images with the convolutional sparse coding method.
 \item Based on the CCSC model, we propose MINet, an interpretable network for UIE. To the best of our knowledge, this is the first model-based interpretable network for the UIE task.
 \item Experiments across two benchmark datasets demonstrate that, with a very low computational complexity, MINet surpasses the state-of-the-art methods.
 \end{itemize}
 

The rest of this paper is organized as follows. Section \ref{sec:method} describes our proposed CCSC model, the architectures of SFEB and MINet, and the loss function in detail. In Section \ref{sec:experiments}, we present extensive experiments to evaluate our method. Finally, we conclude the paper in Section \ref{sec:conclusion}.

==> sec/1_intro1.tex <==
\input{images/fig1}
\section{Introduction}
\label{sec:intro}
Underwater images are essential for various applications, such as marine
biology research, underwater archaeology, and resource management.
However, these images often suffer from severe degradation due to the
absorption and scattering of light in underwater environments. The attenuation
of light is non-uniform across different color channels, exacerbating the issue.
To address these challenges and enhance the usability of underwater images for
high-level vision tasks, numerous underwater image enhancement (UIE)
techniques \cite{uieb,uiewd,scnet,deepwavenet,FUnIEGAN,x_caunet,DSFFNet} have been developed.  Recent methods \cite{deepwavenet,x_caunet} have employed deep neural networks specifically designed for
UIE, considering the non-uniform attenuation of different color wavelengths.
These color channel-specific designs have proven to be highly effective for
UIE. Despite the potential of deep learning (DL)--based methods to learn
complex mappings between degraded and enhanced images, they often lack
interpretability regarding the underlying image enhancement process \cite{unrolling, urolling_boyd}. This
limitation highlights the need for approaches that not only improve image
quality but also provide a clear understanding of the enhancement mechanisms
involved.

To incorporate interpretability in the network architecture, Pham \textit{et al.} \cite{dunet} proposed a deep unfolding network (DUNet) with physics-based priors. They formulated a joint optimization problem for estimating the transmission map and background light in the light scattering model for underwater images \cite{scatter}. To solve this optimization problem, they proposed iterative algorithms based on the alternating direction method of multipliers (ADMM) and then designed a network by unfolding iteration steps. Though DUNet has good interpretability, the inaccuracies in the scattering model limit its performance. Also, \cite{dunet} did not consider the color channel-specific degradation scenario in underwater images.

UIE is an inverse problem, where given a degraded source image $I_s\in\mathbb{R}^{H \times W \times 3}$, the goal is to restore the enhanced image $I_e\in\mathbb{R}^{H \times W \times 3}$. $H$ and $W$ are image height and width, respectively. In the image inverse problems, convolutional sparse coding (CSC)-based models are widely used \cite{csc_cvpr,csc_iccv}. CSC expresses $I_s$ using convolutional sparse representations $z\in\mathbb{R}^{H \times W \times K}$ as,
\begin{equation}\label{eq1}
    I_s = D(z)
\end{equation}

where $D(\cdot)$ is convolutional dictionary which can be learned, and $K$ is number of convolution filters. $z$ is enforced to be sparse by $\ell_1$ norm regularization, and this sparsity helps to highlight the salient features in the input image.

In this work, we propose a novel color channel-specific convolutional sparse coding (CCSC) model to solve the UIE problem. Based on this CCSC model, we propose MINET, a deep network for the UIE task. Due to this model-based design, the architecture of MINET has good interpretability of the underlying image enhancement process.
Specifically, we propose an algorithm unrolling-based sparse feature estimation block (SFEB) to estimate the salient features from the different color channels. Experiments across two benchmark datasets demonstrate that, with very low computational complexity, MINET surpasses the state-of-the-art methods.
 

The rest of this paper is organized as follows. Section \ref{sec:method} describes our proposed CCSC model, the architectures of SFEB and MINET, and the loss function in detail. In Section \ref{sec:experiments}, we present extensive experiments to evaluate our method. Finally, we conclude the paper in Section \ref{sec:conclusion}.

==> sec/4_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

This work introduces SINET, a sparsity-driven interpretable neural network for the underwater image enhancement task. Different from other methods, our network is designed based on a novel channel-specific convolutional sparse coding model. This model-based design provides good interpretability of the underlying image enhancement process. Specifically, SINET estimates the salient features from each color channel using algorithm unrolling-based sparse feature estimation blocks. Our ablation studies justify the design of SINET. 
Experimental results demonstrate that with very low computational complexity, SINET surpasses state-of-the-art methods.
